Fingerprinting Search Keywords over HTTPS at Scale

The possibility of fingerprinting the search keywords issued by a user on popular web search engines is a significant threat to user privacy. This threat has received surprisingly little attention in the network traffic analysis literature. In this work, we consider the problem of keyword fingerprinting of HTTPS traffic -- we study the impact of several factors, including client platform diversity, choice of search engine, feature sets as well as classification frameworks. We conduct both closed-world and open-world evaluations using nearly 4 million search queries collected over a period of three months. Our analysis reveals several insights into the threat of keyword fingerprinting in modern HTTPS traffic.

==> figures/clf_accuracy_type_interval.tex <==
\begin{figure*}[htbp]
\centering
% \vspace{-2mm}
\includegraphics[width=0.95\linewidth]{figures/clf_accuracy_type_interval_fig.pdf}
\vspace{-4mm}
\caption{Impact of typing speed: 9-fold cross-validation accuracy.}
\label{fig:clf_acc_type_interval}
\end{figure*}

==> figures/precision_recall_vary_test.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\linewidth]{figures/precision_recall_vary_test_fig.pdf}
\caption{\emph{Precision-Recall-Curve} achieved with DuckDuckGo using \emph{Wfin++} with 50k non-monitored training samples and varying number of non-monitored testing samples from 0 to around 190k in binary classification scenario.}
\label{fig:precision_recall_vary_test}
\end{figure}

==> figures/search_engine_diff_queries.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=0.95\linewidth]{figures/search_engine_diff_queries_fig.pdf}
\caption{Comparison of network traffic generated for four different monitored search queries (from left to right) searched approximately at the same time with DuckDuckGo and Bing using Chrome. 
% The caption in each sub-figure indicates the searching time: \emph{Year-Month-Day-Hour-Minute-Second}.
}
\label{fig:search_engine_diff_queries}
\end{figure*}

==> figures/time_effect_binary.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.7\linewidth]{figures/time_effect_binary_fig.pdf}
\vspace{-3mm}
\caption{\emph{Average precision}: Impact of Time Gap}
\vspace{-3mm}
\label{fig:time_effect_binary}
\end{figure}

==> tables/bing_top_hostname.tex <==
\begin{table}[htbp]
    \centering
    \caption{List of the top 20 domain names observed in Bing traffic.}
    \begin{tabular}{rrr}
    \hline
    Rank & Second-level hostname & Popularity \\ \hline
        1 & a-msedge.net & 64.83\% \\
        2 & cloudfront.net & 9.46\% \\
        3 & amazonaws.com & 8.91\% \\
        4 & 1e100.net & 3.7\% \\
        5 & akamaitechnologies.com & 2.93\% \\
        6 & ipdns.io & 0.96\% \\
        7 & fastwebserver.de & 0.85\% \\
        8 & dc-msedge.net & 0.63\% \\
        9 & bingforbusiness.com & 0.42\% \\
        10 & ovh.com & 0.39\% \\
        11 & frontiernet.net & 0.35\% \\
        12 & oraclecloud.com & 0.31\% \\
        13 & scalematrix.net & 0.26\% \\
        14 & poneytelecom.eu & 0.21\% \\
        15 & verizon.net & 0.2\% \\
        16 & comcastbusiness.net & 0.13\% \\
        17 & arvixevps.com & 0.12\% \\
        18 & ipvanish.com & 0.12\% \\
        19 & telmex.net.ar & 0.11\% \\
        20 & vnpt.vn & 0.11\% \\
    \hline
    \end{tabular}
    \label{tab:bing_top_hostname}
\end{table}

==> tables/cross_browser_addressbar.tex <==
\begin{table}[H]
    \centering
    \caption{Accuracy (\%) achieved with in cross-browser attack and \emph{addressbar searching} mode.}
    
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{l|cc|cc}
    \hline
    \multirow{2}{*}{\textbf{DDG}} & \multicolumn{2}{c|}{Firefox} & \multicolumn{2}{c}{Chrome} \\ \cline{2-5}
    & \emph{Wfin} & \emph{PSC}  & \emph{Wfin} & \emph{PSC} \\ \hline
    Firefox &  92.87 $\pm$ 0.03&92.44 $\pm$ 0.04  \\ 
    Chrome & & & 96.51 $\pm$ 0.02 & 96.61 $\pm$ 0.02\\
    F/C  & \\ 
    \hline
    
    \multicolumn{5}{c}{} \\ \hline
    
    \multirow{2}{*}{\textbf{Google}} & \multicolumn{2}{c|}{Firefox} & \multicolumn{2}{c}{Chrome} \\ \cline{2-5}
    & \emph{Wfin} & \emph{PSC}  & \emph{Wfin} & \emph{PSC} \\ \hline
    Firefox & 78.44 $\pm$ 0.13 & 79.27 $\pm$ 0.08 &\\ 
    Chrome &  & & 64.05 $\pm$ 0.06 & 59.05 $\pm$ 0.05\\ 
    F/C  & \\ 
    \hline
   
    \end{tabular}
    }
    \label{tab:cross_browser_addressbar}
\end{table}

==> tables/ddg_top_hostname.tex <==
\begin{table}[htbp]
    \centering
    \caption{List of the top 20 domain names observed in DuckDuckGo traffic.}
    \begin{tabular}{rrr}
    \hline
    Rank & Second-level hostname & Popularity \\ \hline
        1 & amazonaws.com & 87.93\% \\
        2 & 1e100.net & 5.35\% \\
        3 & cloudfront.net & 3.5\% \\
        4 & akamaitechnologies.com & 0.33\% \\
        5 & ipdns.io & 0.3\% \\
        6 & fastwebserver.de & 0.27\% \\
        7 & ovh.com & 0.12\% \\
        8 & frontiernet.net & 0.11\% \\
        9 & oraclecloud.com & 0.1\% \\
        10 & scalematrix.net & 0.08\% \\
        11 & poneytelecom.eu & 0.07\% \\
        12 & verizon.net & 0.06\% \\
        13 & arvixevps.com & 0.04\% \\
        14 & comcastbusiness.net & 0.04\% \\
        15 & ipvanish.com & 0.04\% \\
        16 & telmex.net.ar & 0.04\% \\
        17 & datacenter1.com.br & 0.04\% \\
        18 & hinet.net & 0.03\% \\
        19 & hubone.fr & 0.03\% \\
        20 & vnpt.vn & 0.03\% \\
    \hline
    \end{tabular}
    \label{tab:yahoo_top_hostname}
\end{table}

==> tables/gini_mi_accuracy.tex <==
\begin{table}[H]
    \centering
    \caption{Classification accuracy (\%) with two different split criteria.}
    % \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l|cc}
        \hline
        & Gini Index  & Mutual Information \\ \hline
        \emph{PSC} & 92.60 $\pm$ 0.03 & 85.05	 $\pm$ 0.05\\
        \emph{Wfin} & 91.86	$\pm$ 0.07 & 82.90	$\pm$ 0.14\\ 
        \emph{EtResp} &33.16 $\pm$ 0.02 & 30.85 $\pm$ 0.06\\
        \emph{k-FP} & 32.12 $\pm$ 0.06
 & 28.28 $\pm$ 0.10
 \\
        \hline
    \end{tabular}
    % }
    
    \label{tab:gini_index_mi_accuracy}
\end{table}

==> tables/google_top_hostname.tex <==
\begin{table}[htbp]
    \centering
    \caption{List of the top domain names observed in Google/Chrome traffic.}
    \begin{tabular}{rrr}
    \hline
    Rank & Domain name & Popularity \\ \hline
        1 & 1e100.net & 100.0\% \\
        % 1 & 1e100.net & 93.21\% \\
        % 2 & cloudfront.net & 2.41\% \\
        % 3 & amazonaws.com & 1.64\% \\
        % 4 & ipdns.io & 0.21\% \\
        % 5 & fastwebserver.de & 0.2\% \\
        % 6 & akamaitechnologies.com & 0.15\% \\
        % 7 & googleusercontent.com & 0.14\% \\
        % 8 & ovh.com & 0.11\% \\
        % 9 & frontiernet.net & 0.08\% \\
        % 10 & secureserver.net & 0.07\% \\
        % 11 & oraclecloud.com & 0.07\% \\
        % 12 & scalematrix.net & 0.06\% \\
        % 13 & poneytelecom.eu & 0.05\% \\
        % 14 & verizon.net & 0.05\% \\
        % 15 & sl-reverse.com & 0.04\% \\
        % 16 & comcastbusiness.net & 0.03\% \\
        % 17 & hinet.net & 0.03\% \\
        % 18 & telmex.net.ar & 0.03\% \\
        % 19 & ipvanish.com & 0.03\% \\
        % 20 & arvixevps.com & 0.03\% \\
    \hline
    \end{tabular}
    \label{tab:google_top_hostname}
\end{table}

==> tables/hostname_ddg.tex <==
\begin{table*}[htbp]
    \centering
        \caption{Second-level domain name contained in the traffic trace using DuckDuckGo with Chrome.}
    \begin{tabular}{lr|lr|lr|lr}
        \hline
        \multicolumn{2}{l|}{2018-12-30-18-44-25-090412} & \multicolumn{2}{l|}{2018-12-30-19-03-30-693358} &
        \multicolumn{2}{l|}{2018-12-30-19-22-58-211999} &
        \multicolumn{2}{l}{2018-12-30-19-42-11-197768} \\ \hline
        amazonaws.com & 8 & amazonaws.com & 8 & amazonaws.com & 8 & amazonaws.com & 8 \\
1e100.net & 1 & 1e100.net & 1 & 1e100.net & 1 & 1e100.net & 1 \\ \hline
    \end{tabular}
    \label{tab:hostname_ddg}
\end{table*}

==> tables/pesudo_code_httpos.tex <==
\begin{algorithm}
\caption{HTTPOS}
\label{euclid}
% \resizebox{0.95\linewidth}{!}{
\begin{algorithmic}[1]
\State \textbf{Input}: Packet \emph{p: < size of packet (p\_size), direction of packet (p\_direction), time of packet (p\_time)>}
\Procedure{HTTPOS}{}
\If {$p\_direction == \textit{Outgoing}$}
\State $p\_size \gets random.randint(p\_size, MTU)$
\EndIf
\If {$p\_direction == \textit{Incoming}$}
\State $p\_size \gets random.randint(p\_size, 3*MSS)$
\State $n \gets p\_size/MSS $
\State $m \gets p\_size\%MSS$
\For{\texttt{$i=0, i < n, i++$}}
    \State \texttt{<do stuff>}
\EndFor
\EndIf
\State $j \gets \textit{patlen}$
\BState \emph{loop}:
\If {$\textit{string}(i) = \textit{path}(j)$}
\State $j \gets j-1$.
\State $i \gets i-1$.
\State \textbf{goto} \emph{loop}.
\State \textbf{close};
\EndIf
\State $i \gets i+\max(\textit{delta}_1(\textit{string}(i)),\textit{delta}_2(j))$.
\State \textbf{goto} \emph{top}.
\EndProcedure
\end{algorithmic}
% }
\end{algorithm}

==> tables/shared_top_domain_engine.tex <==
\begin{table}[H]
    \centering
    \caption{List of the top shared domains across search engines (\%). }
    \label{tab:top_shared_domains_engine}
    \resizebox{1.0\linewidth}{!}
    {
    \begin{tabular}{rrrrrr}
    \hline
         & Domain name & Google & Bing & Yahoo & DuckDuckGo \\ \hline
        1 & yahoo.com & $<0.01$ & 0.01 & \textbf{34.76} & $<0.01$ \\
        2 & 1e100.net & \textbf{93.21} & 3.7 & 14.84 & 5.35 \\
        3 & amazonaws.com & 1.64 & 8.91 & 15.66 & \textbf{87.93} \\
        4 & fastwebserver.de & 0.2 & 0.85 & 0.04 & 0.27 \\
        5 & a-msedge.net & $<0.01$ & \textbf{64.83} & 1.5 & $<0.01$ \\
        6 & akamaitechnologies.com & 0.15 & 2.93 & 15.93 & 0.33 \\
        7 & ipdns.io & 0.21 & 0.96 & 0.04 & 0.3 \\
        8 & cloudfront.net & 2.41 & 9.46 & 3.5 & 3.5 \\
    \hline
    \end{tabular}
    }
\end{table}

==> tables/specific_domain_chrome.tex <==
\begin{table}[H]
    \centering
    \caption{List of the specific domain names observed in Chrome/Ubuntu 17.10 traffic with more than 0.01\% popularity.}
    \begin{tabular}{rrr}
    \hline
    Rank & Domain name & Popularity \\ \hline
    1 & unifiedlayer.com & 0.01\% \\
    2 & sucuri.net & 0.01\% \\
    3 & ui-r.com & 0.01\% \\
    \hline
    \end{tabular}
    \label{tab:specific_chrome}
\end{table}

==> tables/specific_domain_edge.tex <==
\begin{table}[htbp]
    \centering
    \caption{List of the top 20 specific domain names observed in Edge/Windows 10 traffic with more than 0.01\% popularity.}
    \begin{tabular}{rrr}
    \hline
    Rank & Domain name & Popularity \\ \hline
    1 & ipdns.io & 0.76\% \\
    2 & fastwebserver.de & 0.69\% \\
    3 & ovh.com & 0.31\% \\
    4 & frontiernet.net & 0.27\% \\
    5 & oraclecloud.com & 0.25\% \\
    6 & scalematrix.net & 0.2\% \\
    7 & poneytelecom.eu & 0.17\% \\
    8 & verizon.net & 0.16\% \\
    9 & comcastbusiness.net & 0.1\% \\
    10 & arvixevps.com & 0.1\% \\
    11 & ipvanish.com & 0.1\% \\
    12 & telmex.net.ar & 0.09\% \\
    13 & hinet.net & 0.09\% \\
    14 & datacenter1.com.br & 0.09\% \\
    15 & vnpt.vn & 0.09\% \\
    16 & hubone.fr & 0.08\% \\
    17 & wildpark.net & 0.08\% \\
    18 & scalabledns.com & 0.08\% \\
    19 & ctbctelecom.com.br & 0.08\% \\
    20 & utg.ge & 0.07\% \\
    \hline
    \end{tabular}
    \label{tab:specific_edge}
\end{table}

==> tables/time_effect_binary.tex <==
\begin{table}[]
    \centering
    \caption{AP: Impact of Time (binary classification)}
    \vspace{-3mm}
    \begin{tabular}{|c|cc|cc|}
    \hline
    % \multicolumn{2}{c}{\multirow{2}{*}{220,018}}
    & \multicolumn{2}{c|}{\emph{\small{(Month-Day-Hour-Min)}}} & \multicolumn{2}{c|}{\emph{AP}} \\
    & \emph{Start Time} & \emph{End Time}& \\ \hline
    \emph{train} & 02-27-03-27 & 03-05-19-10 & N/A \\ 
    \emph{test-1} & 03-05-19-11 &03-07-20-15 & \\
    \emph{test-2} & 03-07-20-16 & 03-10-02-07 &\\
    \emph{test-3} & 03-10-02-08 & 03-12-01-10 & \\
    \hline
    \end{tabular}
    \vspace{-3mm}
    \label{tab:time_effect_binary}
\end{table}

==> tables/top_hostname_homepage.tex <==
\begin{table}[htbp]
    \centering
    \caption{List of the top domain names observed in four search engines using Chrome.}
    \begin{tabular}{rrr}
    \hline
    
     \textbf{Rank} & \textbf{Domain name} & \textbf{Popularity} \\ \hline
     \multicolumn{3}{l}{} \\
     \multicolumn{3}{l}{\underline{\textbf{DuckDuckGo}}}  \\
    % \multicolumn{3}{l}{} \\
    
    1 & amazonaws.com & 100.0\% \\
    \multicolumn{3}{l}{} \\
    
    \multicolumn{3}{l}{\underline{\textbf{Google}}}  \\
    % Rank & Domain name & Popularity \\ \hline
    1 & 1e100.net & 100.0\% \\
    
    \multicolumn{3}{l}{} \\
    
    \multicolumn{3}{l}{\underline{\textbf{Bing}}}  \\ 
    % Rank & Domain name & Popularity \\ \hline
    1 & a-msedge.net & 92.73\% \\
    2 & akamaitechnologies.com & 7.27\% \\
    
    \multicolumn{3}{l}{} \\
    
    \multicolumn{3}{l}{\underline{\textbf{Yahoo}}} \\
    
    % \hline
    % Rank & Domain name & Popularity \\ \hline
        1 & yahoo.com & 72.04\% \\
        2 & amazonaws.com & 13.93\% \\
        3 & akamaitechnologies.com & 5.94\% \\
        4 & 1e100.net & 3.87\% \\
        5 & a-msedge.net & 2.55\% \\
        6 & googleusercontent.com & 0.59\% \\
        7 & cdn77.com & 0.39\% \\
        8 & adnexus.net & 0.15\% \\
        9 & openx.org & 0.14\% \\
        10 & doubleverify.com & 0.14\% \\
        11 & zayo.com & 0.11\% \\
        12 & facebook.com & 0.11\% \\
        % 13 & linkedin.com & 0.02\% \\
        % 14 & cloudfront.net & 0.01\% \\
        % 15 & nr-data.net & 0.01\% \\
        % 16 & sl-reverse.com & 0.01\% \\
        % 17 & apxlv.com & 0.0\% \\
        % 18 & hwcdn.net & 0.0\% \\
        % 19 & turn.com & 0.0\% \\
        % 20 & cogocast.net & 0.0\% \\
    \hline
    \end{tabular}
    \label{tab:yahoo_top_hostname}
\end{table}
